Purifying Large Language Models by Ensembling a Small Language Model

The emerging success of large language models (LLMs) heavily relies on collecting abundant training data from external (untrusted) sources. Despite substantial efforts devoted to data cleaning and curation, well-constructed LLMs have been reported to suffer from copyright infringement, data poisoning, and/or privacy violations, which would impede practical deployment of LLMs. In this study, we propose a simple and easily implementable method for purifying LLMs from the negative effects caused by uncurated data, namely, through ensembling LLMs with benign and small language models (SLMs). Aside from theoretical guarantees, we perform comprehensive experiments to empirically confirm the efficacy of ensembling LLMs with SLMs, which can effectively preserve the performance of LLMs while mitigating issues such as copyright infringement, data poisoning, and privacy violations.

==> table4_codellama.tex <==
% Please add the following requiblack packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Experimental results of CodeLlama models facing various levels of copyright violation severity (when $T=0.2$), and \textcolor[HTML]{C0C0C0}{ gray} marks the copyright infringement metrics.
We adjust the ensemble weight $\alpha$, gradually decreasing it from 1.0 to 0, using a decrement interval of 0.2. At \(\alpha\)=1.0, the model is the untrusted LLM; at \(\alpha\)=0, it reflects the benign SLM.
 The symbols \(\uparrow\) and \(\downarrow\) separately indicate whether a higher or lower value of a specific metric is preferable.}
 \vspace{-0.1in}
 \resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c|cccccc}
\toprule
Metrics  & $\alpha$=1.0   & $\alpha$=0.8     & $\alpha$=0.6     & $\alpha$=0.4     & $\alpha$=0.2     & $\alpha$=0     \\
\midrule
pass@1 $\uparrow$  & 0.344 & 0.331 & 0.323 & 0.316 & 0.310 & 0.301 \\
pass@10 $\uparrow$  & 0.524 & 0.518 & 0.506 & 0.482 & 0.468 & 0.458 \\
pass@100 $\uparrow$ & 0.632 & 0.631 & 0.652 & 0.632 & 0.648 & 0.605 \\
\midrule
\colorbox{gray!10}{\strut $\text{IC}_4\downarrow$}   & 0.102 & 0.085 & 0.077 & 0.077 & 0.067 & 0.055 \\
\colorbox{gray!10}{\strut Dolos  $\downarrow$}   & 0.230 & 0.220 & 0.220 & 0.218 & 0.189 & 0.160 \\
\bottomrule
\end{tabular}
}
 \vspace{-0.1in}
\label{tab:extended_exp}
\end{table}

==> table5_bk.tex <==
\begin{table*}[htb]
\caption{Experimental results of Llama2 models when adjusting ensemble weights in generation process to mitigate data poisoning. We adjust the parameter $\alpha$ to 1.0 for generating the first two tokens, and 0.0 for the rest.}
 \vspace{-0.1in}
 \resizebox{2.0\columnwidth}{!}{
\begin{tabular}{cccccc|cccccc}
\hline
\multicolumn{6}{c|}{Standard Performance}                                                                                                                                 & \multicolumn{6}{c}{Severity of Data Poisoning}                                                                                                                               \\ \hline
\multicolumn{1}{c|}{LAMBADA ($T$=0.2)} & \multicolumn{1}{c|}{LogiQA ($T$=0.2)} & \multicolumn{1}{c|}{SciQ} & \multicolumn{1}{c|}{ARC}   & \multicolumn{1}{c|}{PIQA}  & WinoGrande & \multicolumn{1}{c|}{EM ($T$=0.2)} & \multicolumn{1}{c|}{EM ($T$=0.5)} & \multicolumn{1}{c|}{EM ($T$=0.8)} & \multicolumn{1}{c|}{CC ($T$=0.2)} & \multicolumn{1}{c|}{CC ($T$=0.5)} & CC ($T$=0.8) \\ 
\multicolumn{1}{c|}{0.763}         & \multicolumn{1}{c|}{0.403}        & \multicolumn{1}{c|}{0.93} & \multicolumn{1}{c|}{0.784} & \multicolumn{1}{c|}{0.792} & 0.711      & \multicolumn{1}{c|}{8.723}    & \multicolumn{1}{c|}{8.684}    & \multicolumn{1}{c|}{8.252}    & \multicolumn{1}{c|}{0.078}    & \multicolumn{1}{c|}{0.081}    & 0.080    \\ \hline
\end{tabular}
}
 \vspace{-0.1in}
\label{tab:changing_alpha}
\end{table*}

==> tables_interval-0.1/table0.tex <==
\begin{table}[]
\caption{Experimental results of different T settings.}     
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|c|l|l|l|l|l}
\hline
\multicolumn{1}{l|}{StarCoder}                                                     & \multicolumn{1}{l|}{Metrics} & T=0.2 & T=0.4 & T=0.6 & T=0.8 & T=1.0 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Standard\\  Performance\end{tabular}}   & pass@1                       &       &       &       &       &       \\ 
                                                                                   & pass@10                      &       &       &       &       &       \\ 
                                                                                   & pass@100                     &       &       &       &       &       \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Copyright\\  Infringement\end{tabular}} & em                           &       &       &       &       &       \\ 
                                                                                   & dolos                        &       &       &       &       &       \\ \hline
\end{tabular}
}
\label{tab:result_T}
\end{table}

==> tables_interval-0.1/table3_.tex <==
% Please add the following requiblack packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\caption{Experimental results of PII leakage mitigation on Pythia models. We adjust the ensemble weight $\alpha$, gradually decreasing it from 1.0 to 0.0, using a decrement interval of 0.1. At \(\alpha=1.0\), the model is the untrusted LLM; at \(\alpha=0.0\), it reflects the benign SLM.
 The symbols \(\uparrow\) and \(\downarrow\) separately indicate whether a higher or lower value of a specific metric is preferable.}
 \resizebox{2.0\columnwidth}{!}{
\begin{tabular}{cc|c|ccccccccccc}
\toprule
Pythia                                                                              & Metrics                  & $T$   & \multicolumn{1}{c}{$\alpha=1.0$} & \multicolumn{1}{c}{$\alpha=0.9$} & \multicolumn{1}{c}{$\alpha=0.8$} & \multicolumn{1}{c}{$\alpha=0.7$} & \multicolumn{1}{c}{$\alpha=0.6$} & \multicolumn{1}{c}{$\alpha=0.5$} & \multicolumn{1}{c}{$\alpha=0.4$} & \multicolumn{1}{c}{$\alpha=0.3$} & \multicolumn{1}{c}{$\alpha=0.2$} & \multicolumn{1}{c}{$\alpha=0.1$} & $\alpha=0$     \\
\midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}Standard\\  Performance\end{tabular}}   & \multirow{3}{*}{LAMBADA  $\textcolor{black}{\uparrow}$} & 0.2 & 0.624                   & 0.616                  & 0.599                  & 0.581                  & 0.555                  & 0.534                  & 0.504                  & 0.471                  & 0.444                  & 0.412                  & 0.379 \\
&                          & 0.5 & 0.584                   & 0.571                  & 0.556                  & 0.535                  & 0.518                  & 0.488                  & 0.463                  & 0.428                  & 0.402                  & 0.370                  & 0.341 \\
&                          & 0.8 & 0.492                   & 0.479                  & 0.461                  & 0.443                  & 0.423                  & 0.398                  & 0.377                  & 0.347                  & 0.327                  & 0.300                  & 0.270 \\ \cmidrule{2-14} 
& \multirow{3}{*}{LogiQA  $\textcolor{black}{\uparrow}$}  & 0.2 & 0.270                   & 0.259                  & 0.253                  & 0.233                  & 0.238                  & 0.237                  & 0.227                  & 0.214                  & 0.153                  & 0.227                  & 0.009 \\
&                          & 0.5 & 0.277                   & 0.251                  & 0.246                  & 0.237                  & 0.241                  & 0.207                  & 0.227                  & 0.230                  & 0.142                  & 0.237                  & 0.139 \\
&                          & 0.8 & 0.255                   & 0.255                  & 0.246                  & 0.252                  & 0.239                  & 0.203                  & 0.224                  & 0.223                  & 0.105                  & 0.199                  & 0.009 \\ \cmidrule{2-14} 
& SciQ  $\textcolor{black}{\uparrow}$                     & -   & 0.842                   & 0.839                  & 0.825                  & 0.810                  & 0.801                  & 0.789                  & 0.778                  & 0.757                  & 0.727                  & 0.689                  & 0.663 \\ 
& ARC  $\textcolor{black}{\uparrow}$                      & -   & 0.582                   & 0.588                  & 0.588                  & 0.576                  & 0.568                  & 0.554                  & 0.537                  & 0.520                  & 0.496                  & 0.469                  & 0.436 \\ 
& PIQA  $\textcolor{black}{\uparrow}$                     & -   & 0.727                   & 0.723                  & 0.724                  & 0.712                  & 0.702                  & 0.693                  & 0.678                  & 0.671                  & 0.650                  & 0.629                  & 0.619 \\ 
& WinoGrande  $\textcolor{black}{\uparrow}$               & -   & 0.596                   & 0.589                  & 0.585                  & 0.587                  & 0.582                  & 0.589                  & 0.550                  & 0.554                  & 0.537                  & 0.534                  & 0.524 \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Severity of \\ PII Leakage\end{tabular}} & \multirow{3}{*}{EM $\textcolor{black}{\downarrow}$}      & 0.2                                            & 3.651                                           & 3.513                                          & 3.362                                          & 3.228                     & 3.025                     & 2.835                     & 2.552                     & 1.431                     & 0.376                     & 0.026                     & 0.000                     \\
&                          & 0.5                                            & 3.509                                           & 3.390                                          & 3.255                                          & 3.121                     & 2.968                     & 2.778                     & 2.384                     & 1.395                     & 0.456                     & 0.072                     & 0.004                     \\
&                          & 0.8                                            & 3.255                                           & 3.160                                          & 3.045                                          & 2.946                     & 2.829                     & 2.574                     & 2.005                     & 1.095                     & 0.366                     & 0.057                     & 0.007                     \\ \cmidrule{2-14} 
& \multirow{3}{*}{LC $\textcolor{black}{\downarrow}$}      & 0.2                                            & 0.433                                           & 0.410                                          & 0.390                                          & 0.353                     & 0.347                     & 0.307                     & 0.277                     & 0.210                     & 0.063                     & 0.013                     & 0.000                     \\
&                          & 0.5                                            & 0.490                                           & 0.493                                          & 0.457                                          & 0.423                     & 0.387                     & 0.330                     & 0.297                     & 0.277                     & 0.203                     & 0.080                     & 0.017                     \\
&                          & 0.8                                            & 0.497                                           & 0.477                                          & 0.453                                          & 0.413                     & 0.347                     & 0.313                     & 0.303                     & 0.287                     & 0.247                     & 0.117                     & 0.037              \\ 
\bottomrule
\end{tabular}
}
\label{tab:result_pii_appendix}
\end{table*}

==> tables_interval-0.1/table4_.tex <==
% Please add the following requiblack packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\caption{Experimental results of CodeLlama models facing various levels of copyright violation severity (when $T=0.8$).
We adjust the ensemble weight $\alpha$, gradually decreasing it from 1.0 to 0.0, using a decrement interval of 0.1. At \(\alpha=1.0\), the model is the untrusted LLM; at \(\alpha=0.0\), it reflects the benign SLM.
 The symbols \(\uparrow\) and \(\downarrow\) separately indicate whether a higher or lower value of a specific metric is preferable.}
 \vspace{-0.1in}
 \resizebox{2.0\columnwidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
\multicolumn{1}{l}{\textbf{CodeLlama (s=30) }}                                & Metrics                 & \multicolumn{1}{c}{$\alpha=1.0$} & \multicolumn{1}{c}{$\alpha=0.9$} & \multicolumn{1}{c}{$\alpha=0.8$} & \multicolumn{1}{c}{$\alpha=0.7$} & \multicolumn{1}{c}{$\alpha=0.6$} & \multicolumn{1}{c}{$\alpha=0.5$} & \multicolumn{1}{c}{$\alpha=0.4$} & \multicolumn{1}{c}{$\alpha=0.3$} & \multicolumn{1}{c}{$\alpha=0.2$} & \multicolumn{1}{c}{$\alpha=0.1$} & $\alpha=0$     \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Standard \\ performance\end{tabular}}   & pass@1   $\textcolor{black}{\uparrow}$  & 0.287                   & 0.291                  & 0.294                  & 0.292                  & 0.293                  & 0.290                  & 0.289                  & 0.283                  & 0.275                  & 0.265                  & 0.257                 \\
 & pass@10   $\textcolor{black}{\uparrow}$ & 0.666                   & 0.667                  & 0.658                  & 0.661                  & 0.644                  & 0.650                  & 0.646                  & 0.646                  & 0.636                  & 0.612                  & 0.601                 \\
 & pass@100   $\textcolor{black}{\uparrow}$& 0.891                   & 0.882                  & 0.872                  & 0.876                  & 0.882                  & 0.885                  & 0.888                  & 0.884                  & 0.879                  & 0.874                  & 0.873                 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Copyright \\ Infringement\end{tabular}} & EM $\textcolor{black}{\downarrow}$      & 1.519                   & 1.563                  & 1.495                  & 1.406                  & 1.496                  & 1.434                  & 1.405                  & 1.379                  & 1.339                  & 1.307                  & 1.311                 \\
 & Dolos $\textcolor{black}{\downarrow}$   & 0.274                   & 0.256                  & 0.265                  & 0.258                  & 0.251                  & 0.240                  & 0.234                  & 0.216                  & 0.216                  & 0.215                  & 0.199                 \\ \midrule
\multicolumn{1}{l}{\textbf{CodeLlama (s=90) }}                                & Metrics                 & \multicolumn{1}{c}{$\alpha=1.0$} & \multicolumn{1}{c}{$\alpha=0.9$} & \multicolumn{1}{c}{$\alpha=0.8$} & \multicolumn{1}{c}{$\alpha=0.7$} & \multicolumn{1}{c}{$\alpha=0.6$} & \multicolumn{1}{c}{$\alpha=0.5$} & \multicolumn{1}{c}{$\alpha=0.4$} & \multicolumn{1}{c}{$\alpha=0.3$} & \multicolumn{1}{c}{$\alpha=0.2$} & \multicolumn{1}{c}{$\alpha=0.1$} & $\alpha=0$     \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Standard \\ performance\end{tabular}}   & pass@1   $\textcolor{black}{\uparrow}$  & 0.286                   & 0.290                  & 0.294                  & 0.298                  & 0.294                  & 0.291                  & 0.288                  & 0.283                  & 0.276                  & 0.268                  & 0.257                 \\
 & pass@10   $\textcolor{black}{\uparrow}$ & 0.654                   & 0.652                  & 0.664                  & 0.664                  & 0.653                  & 0.658                  & 0.648                  & 0.639                  & 0.630                  & 0.620                  & 0.601                 \\
 & pass@100   $\textcolor{black}{\uparrow}$& 0.878                   & 0.878                  & 0.884                  & 0.890                  & 0.870                  & 0.887                  & 0.883                  & 0.878                  & 0.889                  & 0.868                  & 0.873                 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Copyright \\ Infringement\end{tabular}} & EM $\textcolor{black}{\downarrow}$      & 23.430                  & 21.692                 & 19.383                 & 15.928                 & 11.726                 & 7.433                  & 4.540                  & 3.051                  & 2.270                  & 1.715                  & 1.311                 \\
 & Dolos $\textcolor{black}{\downarrow}$   & 7.696                   & 7.328                  & 6.806                  & 5.834                  & 4.337                  & 2.582                  & 1.244                  & 0.648                  & 0.389                  & 0.274                  & 0.199                 \\ \bottomrule
\end{tabular}
}
 \vspace{-0.1in}
\label{tab:extended_exp_appendix}
\end{table*}
